Relative entropy of coherent states on general CCR algebras

For a subalgebra of a generic CCR algebra, we consider the relative entropy between a general (not necessarily pure) quasifree state and a coherent excitation thereof. We give a unified formula for this entropy in terms of single-particle modular data. Further, we investigate changes of the relative entropy along subalgebras arising from an increasing family of symplectic subspaces; here convexity of the entropy (as usually considered for the Quantum Null Energy Condition) is replaced with lower estimates for the second derivative, composed of "bulk terms" and "boundary terms". Our main assumption is that the subspaces are in differential modular position, a regularity condition that generalizes the usual notion of half-sided modular inclusions. We illustrate our results in relevant examples, including thermal states for the conformal $U(1)$-current.

==> macros.tex <==
% Layout definitions


% ``Details'' environments and commands
\RequirePackage{color}
\definecolor{detailsgray}{gray}{0.3}

\makeatletter
\@ifundefined{showdetailstrue}{\newif\ifshowdetails
\showdetailstrue}{}
\makeatother

\ifshowdetails
\newcommand{\detail}[1]{%
{\color{detailsgray}$\blacktriangleright${#1}$\blacktriangleleft$}%
}

\newcommand{\detailspar}[1]{
\par \noindent {\color{detailsgray} $\blacktriangleright$ \textit{#1} $\blacktriangleleft$ } \par
}

\newenvironment{details}{\par \noindent \begingroup\itshape\color{detailsgray} $\blacktriangleright$ \hrulefill%
\par \noindent \ignorespaces}{\par\noindent \hrulefill $\blacktriangleleft$  \endgroup \par \noindent}

\else
\newcommand{\detail}[1]{} 
\newcommand{\detailspar}[1]{} 
\usepackage{environ}
\NewEnviron{hide}{}
\let\details\hide
\let\enddetails\endhide

\fi


% Makrodefinitionen (global)


\def \cbb{\mathbb{C}}
\def \ibb{\mathbb{I}}
\def \nbb{\mathbb{N}}
\def \rbb{\mathbb{R}}
\def \qbb{\mathbb{Q}}
\def \zbb{\mathbb{Z}}

\def \acal {\mathcal{A}}
\def \bcal {\mathcal{B}}
\def \ccal {\mathcal{C}}
\def \dcal {\mathcal{D}}
\def \ecal {\mathcal{E}}
\def \fcal {\mathcal{F}}
\def \gcal {\mathcal{G}}
\def \hcal {\mathcal{H}}
\def \ical {\mathcal{I}}
\def \jcal {\mathcal{J}}
\def \kcal {\mathcal{K}}
\def \lcal {\mathcal{L}}
\def \mcal {\mathcal{M}}
\def \ncal {\mathcal{N}}
\def \ocal {\mathcal{O}}
\def \pcal {\mathcal{P}}
\def \qcal {\mathcal{Q}}
\def \rcal {\mathcal{R}}
\def \scal {\mathcal{S}}
\def \tcal {\mathcal{T}}
\def \ucal {\mathcal{U}}
\def \vcal {\mathcal{V}}
\def \wcal {\mathcal{W}}
\def \xcal {\mathcal{X}}
\def \ycal {\mathcal{Y}}
\def \zcal {\mathcal{Z}}

\def \afk  {\mathfrak{A}}
\def \bfk  {\mathfrak{B}}
\def \dfk  {\mathfrak{D}}
\def \ffk  {\mathfrak{F}}
\def \lfk  {\mathfrak{L}}
\def \mfk  {\mathfrak{M}}
\def \nfk  {\mathfrak{N}}
\def \pfk  {\mathfrak{P}}
\def \qfk  {\mathfrak{Q}}
\def \vfk  {\mathfrak{V}}
\def \wfk  {\mathfrak{W}}
\def \xfk  {\mathfrak{X}}
\def \zfk  {\mathfrak{Z}}

\newcommand{\betav}{\boldsymbol{\beta}}
\newcommand{\thetav}{\boldsymbol{\theta}}
\newcommand{\etav}{\boldsymbol{\eta}}
\newcommand{\lambdav}{\boldsymbol{\lambda}}
\newcommand{\nuv}{\boldsymbol{\nu}}
\newcommand{\zetav}{\boldsymbol{\zeta}}
\newcommand{\piv}{\boldsymbol{\pi}}
\newcommand{\xiv}{\boldsymbol{\xi}}

\newcommand{\av}{\mathbf{a}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\ev}{\mathbf{e}}
\newcommand{\nv}{\mathbf{n}}
\newcommand{\pv}{\mathbf{p}}
\newcommand{\qv}{\mathbf{q}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\zv}{\mathbf{z}}
\newcommand{\zerov}{\mathbf{0}}

\newcommand{\xn}{\lvert\boldsymbol{x}\rvert}

% Spacing

\def \. { \,\! }

\def\clap#1{\hbox to 0pt{\hss#1\hss}}
\def\mathllap{\mathpalette\mathllapinternal}
\def\mathrlap{\mathpalette\mathrlapinternal}
\def\mathclap{\mathpalette\mathclapinternal}
\def\mathllapinternal#1#2{\llap{$\mathsurround=0pt#1{#2}$}}
\def\mathrlapinternal#1#2{\rlap{$\mathsurround=0pt#1{#2}$}}
\def\mathclapinternal#1#2{\clap{$\mathsurround=0pt#1{#2}$}}

\def \cdotarg { \, \cdot \, }

% Operators

\DeclareMathOperator{\im}{Im}
\DeclareMathOperator{\re}{Re}

\newcommand{\id}{\operatorname{id}}
\newcommand{\idop}{\boldsymbol{1}}

\def \half {\frac{1}{2}}

\def \csq {\quad \Rightarrow \quad}

\def \into {\rightarrow}
\def \st {^\ast}
\def \isom {\cong}
\newcommand{\restrict}{\restriction}

\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\img}{img}

\newcommand{\dalembert}{\Box}

\def \noqed{ \renewcommand{\qed}{} }


\newcommand{\etskp}[2]{\langle #1 | #2 \rangle }

%%% Operator spaces and vector spaces

% Hilbert space (Fock space)
\newcommand{\Hil}{\mathcal{H}}

% Z spaces
\newcommand{\z}{\mathcal{Z}}
\newcommand{\zb}{\bar{\mathcal{Z}}}


% Space of vectors of finite particle number
\newcommand{\fpn}{\Hil^{\mathrm{f}}}
\newcommand{\fpno}{\Hil^{\omega,\mathrm{f}}}
\newcommand{\fpnp}{P^{\mathrm{f}}}


% Bounded operators on H
\newcommand{\boundedops}{\bfk(\Hil)}

% Quadratic forms
\newcommand{\qf}{\mathcal{Q}}

% (Local) algebra in general
\newcommand{\A}{\mathcal{A}}
% Standard wedge algebra 
\newcommand{\M}{\mathcal{M}}

% Hilbert space (Fock space) scalar product - three different sizes
\newcommand{\hscalar}[2]{\langle #1 , #2 \rangle }
\newcommand{\bighscalar}[2]{\big\langle  #1 , #2 \big\rangle }
\newcommand{\Bighscalar}[2]{\Big\langle  #1 , #2 \Big\rangle }

% Norms for quadratic forms
\newcommand{\qfnorm}[2]{\lVert #1 \rVert_{#2}}

% Generic norm with subscript
\newcommand{\gnorm}[2]{\lVert #1 \rVert_{#2}}
\newcommand{\biggnorm}[2]{\big\lVert #1 \big\rVert_{#2}}
\newcommand{\Biggnorm}[2]{\Big\lVert #1 \Big\rVert_{#2}}
% Omega norm with subscript
\newcommand{\onorm}[2]{\lVert #1 \rVert_{#2}^\omega}
\newcommand{\bigonorm}[2]{\big\lVert #1 \big\rVert_{#2}^\omega}
\newcommand{\Bigonorm}[2]{\Big\lVert #1 \Big\rVert_{#2}^\omega}

% distributional pairing
\newcommand{\dev}[2]{ \left\langle #1, #2 \right\rangle }

%%% Geometrical regions

\newcommand{\leftwedge}{\mathcal{W}'}
\newcommand{\rightwedge}{\mathcal{W}}

%%% Miscellaneuous symbols

% a,z dagger
\newcommand{\ad}{a^\dagger}
\newcommand{\zd}{z^\dagger}
\newcommand{\adpm}{a^\dagger_\pm}
\newcommand{\apm}{a_\pm}

% left and right ``vector'' distributions
\newcommand{\lvector}[2]{\boldsymbol{\ell}_{#1}(#2)}
\newcommand{\rvector}[2]{\boldsymbol{r}_{#1}(#2)}

% contracted matrix element
\newcommand{\cmeA}[2]{f_{#1}^{\lbrack #2 \rbrack}}
\newcommand{\cmeB}[2]{f_{#1}{\lbrack #2 \rbrack}}
\newcommand{\cme}[2]{\mathchoice{\cmeA{#1}{#2}}{\cmeB{#1}{#2}}{\cmeB{#1}{#2}}{\cmeB{#1}{#2}}}
\newcommand{\cmelong}[2]{f_{#1} \left\lbrack #2 \right\rbrack}

% analytic indicatrix
\newcommand{\oa}{\varpi}

% strip in the complex plane
\DeclareMathOperator{\strip}{S}

% ``affiliated with'' relation
\newcommand{\affiliated}{\mathrel{\eta}}

% tube over a set
\newcommand{\tube}{\mathcal{T}}

% Symmetric group; Sign of a permutation
\newcommand{\perms}[1]{\mathfrak{S}_{#1}}
\DeclareMathOperator{\sign}{sign}

% residue
\DeclareMathOperator*{\res}{res}

% domain
\DeclareMathOperator*{\domain}{dom}

% various functions
\DeclareMathOperator{\arcoth}{arcoth}

% upper index (for polynomials etc)

\newcommand{\uidx}[1]{^{\lbrack #1 \rbrack}}
\newcommand{\lidx}[1]{_{ #1 }}

% even/odd

\newcommand{\even}{^\mathrm{even}}
\newcommand{\odd}{^\mathrm{odd}}

% power sum polynomial
\newcommand{\psp}[1]{\pi_{#1}}

\newcommand{\inv}{_\mathrm{I}}

\newcommand{\expect}[2]{\left\langle #1 \right\rangle_{#2}}

\newcommand{\nosq}{ {:} \phi^2 {:}}

\newcommand{\relent}[3]{S_{#3}({#1 {\parallel} #2})}

% ``purified'' object
\newcommand{\pf}{^{\oplus}}
\newcommand{\ipf}{\imath^\oplus}

% abelian, factorial, etc. subscripts
\newcommand{\fact}{\mathsf{f}}
\newcommand{\abel}{\mathsf{a}}
\newcommand{\std}{\mathsf{s}}

% ccr algebra
\DeclareMathOperator{\ccr}{CCR}

% Entropy space
\newcommand{\es}{\mathcal{X}}

% spectrally cut domain
\newcommand{\dcut}{\dcal^{(0)}}


